A State-Based Regression Formulation for Domains with Sensing Actions<br> and Incomplete Information

We present a state-based regression function for planning domains where an agent does not have complete information and may have sensing actions. We consider binary domains and employ a three-valued characterization of domains with sensing actions to define the regression function. We prove the soundness and completeness of our regression formulation with respect to the definition of progression. More specifically, we show that (i) a plan obtained through regression for a planning problem is indeed a progression solution of that planning problem, and that (ii) for each plan found through progression, using regression one obtains that plan or an equivalent one.

==> lmcs-review <==
Response to comments of the reviewers:

Referee no 2:

 * The paper can be accepted for Logical Methods in Computer Science after minor revisions.

Recommendation: The paper can be accepted for Logical Methods in
Computer Science after minor revisions. Further refereeing is not necessarily needed.

-------------------

The paper studies the notion of regression in the setting of
STRIPS-like planning where states represent the knowledge acquired by
the agent instead of truth in the world.

The result reported are novel and worth publishing. Also the technical
part of the paper is well written, and the proof arguments reported are
convincing.

The paper, in the current version however is not self contained enough
and essentially requires the reader to first read [16] ("T.C.Son and
C. Baral, Formalizing sensing actions, AIJ 125(1-2), Jan 2001"), in order to
understand the context in which the result is obtained.

I suggest the authors to make an effort so that the paper can be read
and understood on its own.



In order to do so the author should:

1. Rewrite the introduction so to introduce the progression-based semantics
on intuitive grounds without referring to 0-approximations;

2. Rewrite Section 2.2 to formally give the progression-based semantics,
again without referring to 0-approximations;

3. Add a section that put the semantics introduces into context wrt
[16] and relates it to 0-approximations;

4. Adjust the Conclusion in light of these changes.

The Introduction (Section 1) should be rewritten so as to avoid
referring to the notion of 0-approximation semantics. Instead the
progression-based semantics should be introduced on intuitive grounds here
without referring to previous work (notice that the semantics has a
perfectly clear appeal on its own and not as a approximation for
something else.

As a result of this the Introduction will almost certainly need to
expanded of roughly 1 page. But I don't think this is a problem in
fact the introduction in the current version is very short.

>>> We rewrote the introduction as suggested.

Along the same line in Section 2.2 instead of simply reporting the
technical definition of 0-approximation, the authors should give in
formal terms and discuss the progression-based semantics again
starting from first principles. I expect this section to grow as
well. But again this is perfectly fine.

>>> We rewrote this section as suggested.

Once the semantics is given then a discussion that relates such a
progression-based semantics (by know perfectly justified on intuitive
and formal ground) to 0-approximations of [16]. I expect such a
section to be more that a simple reference to [16] plus the
observation that the progression-based semantics given here is a
synonyms of 0-approximations. Instead I expect such a section to
explain on intuitive grounds kind of approximation wrt [16] the
progression-based semantics is, referring to [16] only for the
technical results.

>>> We added the section on the property of the progression function
    (Section 2.3).

>>> We reworded the conclusion.

Additional and minor comments:

1. For clarity don't assume that the setminus operation has precedence
over union. Use parenthesis instead (eg. page 5, line -5).

>>> We did this.

2. In LaTex, the string "ff" in math mode looks strange use \mathit
instead (eg, page 6, line +3).

>>> We did this.

3. Page 7, line +23: "it is extended to ..." it is unclear to whom
"it" refers to.

>>> We reworded the sentence to make it clear.

4. Applicability conditions --&#62; Regression applicability condition (eg
Definition 4, Definition 8, Definition 9)

>>> We added 'Regression' to the names of the definition whereever we
    find it is appropriate/

5. Definition 6. Such a definition is very technical. Please give more
intuition on what p(a \Delta) is and why can be defined in that way.

>>> We added a discussion after the definition to elaborate more on
    the intuition behind the notion p(a,\Delta).

6. Definition 13. This is the core notion of the paper. After having
given it you should discuss in same length (say at least half a
page). In particular: why we care about regression solutions? What is
their conceptual/theoretical/pragmatical significance? Are they better
(in any sense) to progression solutions? You say something in the
conclusion but you should say more here (as well as anticipating the
main points of the discussion in the Introduction).

>>> We added a discussion.

7. In the related work you may consider to say something more on the
work on weakest preconditions on nondeterministic programs (as for
your plans with sensing). A nice treatment can be found, for example,
in chapter 3 of "Eike Best, Semantics of Sequential and Parallel
Programs, Prentice Hall, 1996".

>>> We added the reference and another reference *de Bakker*.

8. In the conclusion please put in relation the Bylander's
PSPACE-completeness of planning in STRIPS with the complexity results
that you mention.

Bylander, T. 1994. The computational complexity of propositional
STRIPS planning. Artificial Intelligence 69(1-2):165-204.

>>> We added the reference.

Referee no 1:

 * The paper can eventually be accepted for Logical Methods in Computer 
Science. I suggest resubmission.

Based on an existing progression function for conditional plans with sensing
actions, the authors define a regression operator. The main result is a
soundness and completeness theorem relating the two problem solution methods.
In the light of earlier work, the paper is moderately, but sufficiently,
original and significant; however, the technical result is flawed, see below.
I therefore recommend resubmission of a corrected version and a second round
of reviewing.

Detailed comments:

The completeness result (Theorem 4) is flawed. Its prrof relies on Lemma 15,
which claims that for any progression solution a regressable plan can be
constructed. This, however, is not true. A counterexample is the following
planning problem, a slight modification of Example 11:

  A = {f,g,h}
  O = {a,b,c}
  I = {h}
  G = {g}

along with the action sepcification

  Pre_a = {f}  Add_a = {g}   Del_a = {}
  Pre_b = {-f} Add_b = {g}   Del_b = {}
  Pre_c = {}   Sens_c = {f,h}

Then p := c; f->a, -f->b is a progression solution. On the other hand, this
plan is not a regression solution because

  R*(p,[{g},{}]) = R(c,{[{f},{}], [{},{f}]}) = false

(since Sens_c is not known in {[{f},{}], [{},{f}]}). But also the plan
p' := c; {f,h}->a, {-f,h}->b, constructed according to Lemma 14, is not
regressable because it is redundant, as can be seen with the subplan
p'' := subSense(c); {f,h}->a, {-f,h}->b (where subSense(c) only senses f).

Tracing the proof for Lemma 15 with this counterexample shows where the
omission lies: The plan p' constructed in paragraph (1)(b) may in fact be
redundant, contrary to what is being claimed.


>>> Thank you very much for this comment. We slightly modified the
    notion of redundancy to addresses this problem. Below, we discuss 
    the main idea of the new definition.  

>>>>>>>>>>>>>>>>>

First, let us repeat here the construction in Lemma 14

For the plan: a; case(\varphi_1->p1;...;\varphi_n->pn) and a-state \sigma:

- we identify what fluents are really sensed by the sensing action
        Sens_a
  this will be the fluents in Sens_a which are unknown in \sigma. 
  (In the paper, this set is denoted by S_a) 

  In your example: this is {f} 

- we then generate the conditions to cover all the possible a-states that 
  are contained in \Phi(a, \sigma) - each of this condition consists of 
  three parts: 
        + condition characterizing an interpretation of 
                Sens_a \setminus \sigma            
                (in the paper: \nu_i^j)
		    (in your example: f and -f) 	
        + condition from \varphi_i which is true in \sigma 
                (in the paper: \varphi)
                (in your example: true)
        + condition that characterizes what belong to Sens_a and are known 
          in \sigma
		    (in your example: h)
 
* this construction makes sure that we cannot replace the *new* plan by 
any of its branches; we cannot remove any branch as well.

Our mistake in the original paper lies in that we should have replaced 
a with subSense(Sens_a \setminus \sigma) after the construction.  

We could have done so and kept the original definition of redundancy.

However, we observed that we can as well keep the action a (since it does 
indeed generate some new knowledge). To do so, we removed the part 
on replacing a by some subSense(a) in the paper and introducing 
the case (iii) in the definition of redundancy to cover the case where 
no new knowledge is added due to the execution of action a (i.e., when
S_a = \emptyset). 

We prefer the new definition since it is simpler than the old one and it 
does not introduce new actions to the original theory. 

>>>>>>>>>>>>>>>>>

Further comments and suggestions:

The authors frequently write of "to regress an action". They should stick to
the standard terminology according to which states (or formulas) are
regressed (through actions).

>>> We changed to 'regress over an action from a state/formula' throughout
    the paper.

I recommend not to use Latex's math mode (which adds a small space in between
two consecutive letters) for literals like "traffice-bad".

>>> We replaced with 'mathit' following the suggestion of the other reviewer.

The last but one sentence on page 8 should be removed, since according to
Lemma 1 there is always a unique subset of Sens_a that satisfies the condition
of Definition 6.

>>> We removed it.

Page 10, line 5f: "we will receive a p_state extending the initial p-state".
This should be the other way round.

>>> We corrected it.

Page 11, paragraph prior to Definition 12: Instead of saying that phi is an
(arbitrary) fluent formula, it would be simpler to write "For a conjunction
of fluent literals phi, by phi+ and phi- we denote...".

>>> We corrected it.

I suggest to replace, in Definition 12, R(c_i,delta) by, say,
R(phi_i->c_i, delta), because the function also depends on phi_i.

>>> We did this.

In Definition 13, the condition described in the last two lines can be
simply stated as "<I+,I-> in ext(R*(c,delta_G))."

>>> We changed this.

In Examples 11 and 12, the set O should be {b,c} instead of {a,b}.

>>> We corrected this.

In Definition 15, item (i) (and elsewhere) the condition "false not-in
Phi*(c,sigma)" can be omitted because it follows from the second condition,
"Phi*(c,sigma) subset ext(delta)."

>>> We made this change throughout the paper.

Definitions 17 and 18 are referred to only in the proof of Theorem 4. Hence,
they should be moved to the appendix. It took me some time to understand
the motivation behind the introduction of BIN(S) etc. I recommend to add
some explanatory remarks. Also, the authors may consider to replace the
notion of "possibly regressable" by "potentially regressable."

>>> We did the above.

In the second paragraph of the proof for Lemma 1, it is simpler to say that
X and X' are non-empty by Definition 6. In the fourth paragraph, it would help
to add "item (4)" after "Definition 6."

>>> We did this.

Given the "without loss of gnereality"-assumption earlier in the proof, the
third and fourth lines on page 20 are superfluous.

>>> We removed the two lines.

The phi_i' in line 11 on page 31 should be phi_j'.

>>> We corrected this.

